Hikester - the event management application

Today social networks and services are one of the most important part of our everyday life. Most of the daily activities, such as communicating with friends, reading news or dating is usually done using social networks. However, there are activities for which social networks do not yet provide adequate support. This paper focuses on event management and introduces "Hikester". The main objective of this service is to provide users with the possibility to create any event they desire and to invite other users. "Hikester" supports the creation and management of events like attendance of football matches, quest rooms, shared train rides or visit of museums in foreign countries. Here we discuss the project architecture as well as the detailed implementation of the system components: the recommender system, the spam recognition service and the parameters optimizer.

==> conclusion.tex <==
\section{Conclusion}



==> mobile_apps.tex <==
\subsection{Mobile Applications}
The key task of developing a mobile application is to make the most simple, convenient and user-friendly interface for the user. The connection with the back-end will be maintained using the JSON API. The main design pattern on which mobile apps will be built is based on is VYPER: View, Interactor, Presenter, Entity, and Routing. That pattern allow to develop applications on high level of abstraction. Separating application on several different and independent part will provide to more easily support in future. 

==> webapp.tex <==
\subsubsection{Web Application}
Web part of Hikster represented as a single page web application[11, 12].
The logic of the front-end will be made on the JavaScript, using the reactJS
framework[13], and the web application state control system - REDUX. ReactJS
based on its own state model[14]. Concept of state is taken from state
machine, there state is some set of variable of some virtual DOM element in
certain moment of time. And changing state of each page element allows to
change some part of page without reloading, because of that there is single
page application. The connection with the back-end will be implemented
via JSON API using a third-party FETCH library. To support liquid architecture,
another important criterion for constructing the frontend was the
availability of responsive design.
